A Mixture of Expert Approach for Low-Cost Customization of Deep Neural Networks

The ability to customize a trained Deep Neural Network (DNN) locally using user-specific data may greatly enhance user experiences, reduce development costs, and protect user's privacy. In this work, we propose to incorporate a novel Mixture of Experts (MOE) approach to accomplish this goal. This architecture comprises of a Global Expert (GE), a Local Expert (LE) and a Gating Network (GN). The GE is a trained DNN developed on a large training dataset representative of many potential users. After deployment on an embedded edge device, GE will be subject to customized, user-specific data (e.g., accent in speech) and its performance may suffer. This problem may be alleviated by training a local DNN (the local expert, LE) on a small size customized training data to correct the errors made by GE. A gating network then will be trained to determine whether an incoming data should be handled by GE or LE. Since the customized dataset is in general very small, the cost of training LE and GN would be much lower than that of re-training of GE. The training of LE and GN thus can be performed at local device, properly protecting the privacy of customized training data. In this work, we developed a prototype MOE architecture for handwritten alphanumeric character recognition task. We use EMNIST as the generic dataset, LeNet5 as GE, and handwritings of 10 users as the customized dataset. We show that with the LE and GN, the classification accuracy is significantly enhanced over the customized dataset with almost no degradation of accuracy over the generic dataset. In terms of energy and network size, the overhead of LE and GN is around 2.5% compared to those of GE.

==> MOE-boyu.tex <==
\vspace{-2mm}
\section{Design Methodology and Architecture of MOE}\label{sec:moe}

\begin{figure}[t]
        \centering
        \includegraphics[width=2in]{figs/moe.pdf}\vspace{-3mm}
        \caption{Diagram of the MOE architecture}\vspace{-7mm}
        \label{fig:moe}
\end{figure}

A block diagram of the proposed MOE architecture is shown in Fig. \ref{fig:moe}. It consists of a global expert (GE), one or more local experts (LEs), and a gating network (GN) that provides a data dependent \textcolor{black}{selection signal to select the output of either} the GE or one of the LEs. In the case of multiple LEs, each one may represent one class of users. Ideally, if the GE provides a correct output with respect to a given input, the GN will just pass through GE's output as the final output and suppress LE's output. If an LE is more likely to provide a correct output, then the output of the GE (and other LEs) will be suppressed. Therefore, the GN plays a central role in the MOE architecture. For each input feature vector, it predicts which of the experts (GE and LEs) is more likely to provide a correct output and then connect the output of that expert to the final output. In this manner, the GN behaves like an intelligent multiplexer, multiplexing the outputs of GE and LEs according to the predicted likelihoods of their output to be correct. For simplicity, we only discuss the case with one LE in the subsequent sections but the discussions can be easily extended to more than one LE.

% Fig. \ref{fig:moe} shows the diagram of the proposed MOE architecture. In its most general form, it consists of three components: one global expert (GE), one or more local experts (LEs), and one gating network (GN). If in case of multiple LEs, each one may represent one class of users. For any given input sample, the GE and all LE(s) will perform classification on it and generate their outputs. Then one of these outputs is selected by GN to be the final output of the entire model. Conceptually, GN provides the selection signal for a multiplexer, which is used to select the final output from the outputs generated by GE and all LE(s). In the following subsections, we first go through the details of these three components. Then we discuss the hardware overheads associated with LE(s) and our proposed architecture optimization techniques to alleviate those overheads. Finally, we talk about the value of LE(s) to and GE, how it can be measured, why the LE(s) are able to improve the overall performance intuitively. For simplicity, we only discuss the case with one LE in the subsequent sections but the discussions can be easily extended to more than one LE.

\vspace{-2mm}
\subsection{Details of the Three Components in MOE}\label{sec:threecomponents}

\noindent \textbf{Global Expert:} We envision there will be an IP (intellectual property) market for trained DNN on very large generic dataset. These carefully designed and trained DNNs may be licensed by vendors to be incorporated into intelligent cognitive devices to facilitate speech recognition, face recognition, and other intelligent services. These trained DNNs will be designated as the Global Expert (GE). The weight values and internal structures are proprietary information and cannot be revealed to or modified (re-trained) by individual users. Therefore, given an input feature vector, a GE will provide the corresponding output, and corresponding internal neural outputs (e.g., extracted features) to the user, but cannot be retrained at the embedded device. Since the GE is trained with generic dataset, it is expected to make a few mistakes on customized data. The users may then opt to provide these mistakenly classified customized data back to the vendor. As such, the vendor may further design and train the GE to improve its performance. Then the updated GE is released to users as a firmware update. However, such an update is expected to be a rare event and can be disabled if the communication with cloud is unavailable. %Moreover, such update will likely aggregate multiple users' feedback to make it usable for a larger user audience while not violating users' data privacy concerns.

% A GE may be updated by the vendor and installed on the embedded device

% \noindent \textbf{Global Expert:} GE is a DNN that is designed and trained by a vendor based on the generic dataset. Thus, it may be licensed from the vendor in the form of an intellectual property (IP) and hence its content (DNN structure or/and weight values) may not be completely transparent to users. However, we assume in some cases, it will provide outputs not only at the final layer but potentially from earlier layers in the form of intermediate features extracted by GE from the input data. Since the GE is trained with generic dataset, it is expected to make a few mistakes on customized data. The users may then opt to provide the customized data that cannot be correctly processed by GE back to the vendor. As such, the vendor may further design and train the GE to recognize more features and improve the performance of GE. Then the updated GE is released to customer just like current software application updates. Moreover, such vendor-based update will aggregate multiple users' feedback to make it usable for a larger user audience while not violating users' data privacy concerns. We also note that this kind of update of GE is just an optional feature, and it can be disabled if the communication with cloud is unavailable.

\noindent \textbf{Local Expert:} A Local Expert (LE) is a local trainable DNN residing within the intelligent cognitive device. It will be trained on a small size local customized dataset with the purpose to generate correct result when presented with customized data. The customized training dataset is collected by the system during daily uses.
% \textcolor{blue}{, and the corresponding ground truth labels are provided by the user implicitly (when user accept the system's output) or explicitly (when user manually correct the system's output)}.
Since the size of the customized dataset is much smaller than that of the generic dataset, LE would have a much smaller and simpler DNN structure compared to that of the GE. This lightweight structure incurs less hardware overhead, which is critical for deploying the entire system on embedded and mobile platforms. Moreover, because both the customized dataset and the LE are small, the training of LE can be easily carried out by software or co-processor on-chip.

% \noindent \textbf{Local Expert:} The purpose of LE is to correctly classify customized data, regardless of whether GE is able to do it or not. Thus, LE will be a much smaller DNN or other lightweight machine learning model because of two reasons: 1) the size of the customized dataset is much smaller than that of the generic dataset, which suggests a lightweight model may be sufficient for classifying the custom data, and at the same time avoid overfitting issue; 2) lightweight model incurs less hardware overhead, which is critical for deploying the entire system on embedded and mobile platforms. LE is trained with customized data, which has the same set of labels as those of the generic data and is provided by users after deployment. Since both the size of customized data and LE are small, the training of LE does not require extensive computation resources and could be easily carried out by software or co-processor on-chip.

\noindent \textbf{Gating Network:} In this work, GN's task is to select the output generated by either GE or LE, and use it as the final output. More generally, GN can be viewed to have two outputs: $w_G$, and $w_L$ such that $0\leq w_G$, $w_L\leq 1$, and $w_G + w_L = 1$. The outputs of GE and LE will be weighted by $w_G$, and $w_L$ respectively. The gating network (GN) will then act as a mediator between the GE and the LE: If it is likely the GE will provide the correct answer, then $w_G >> w_L$, meaning the GE's output will be selected as the final output. On the other hand, if it is more likely that the LE's output is correct, then $w_G << w_L$ meaning the LE's output will be the final output.  



%It acts as a mediator between the GE and the LE: when $w_G \geq w_L$, the GE's output will be selected as the final output. On the other hand, if $w_G < w_L$, then the LE's output will be the final output. The GN is trained with equal number of samples that instruct GN to choose GE (with label $w_G=1, w_L=0$) or LE (with label $w_G=0, w_L=1$). 

There are two possible approaches for training the GN. In the first approach, GN is trained to predict if GE is able to provide correct output for the given input data (whether generic or customized), then select the output of GE if the prediction from GN is true. Otherwise, select the output of LE only for those customized data that are not predicted correctly by GE.  The issue that we observed with this approach in our implementation is that, the number of samples in customized dataset that instruct GN to select the output from LE will be smaller, for example about 25\% of the customized dataset as we studied in our experiments. As a result, GN may not receive enough training samples and cannot be trained properly to identify which output should be selected.

Due to the above issue we used the following alternative approach: Here, GN predicts if the input data is more likely to be from the generic or customized dataset. It then selects the output of GE or LE accordingly. Thus, GN is trained with all customized data plus equal number of randomly sampled generic data. The number of generic data required for training of GN is very small, for example only about 1\% of the size of the generic dataset in our experiments. Therefore the small number of generic data required for the training of GN can be pre-loaded in the system or downloaded from cloud if network connection is available. Overall, similar to LE, we expect GN to be lightweight and its training can be carried out by software or a co-processor.% We implemented both approaches in our experiments and confirmed the second one indeed performs better.

\vspace{-3mm}
\subsection{Optimization of LE and GN Architecture}
\vspace{-1mm}
LE and GN are expected to be lightweight and for example, for the image classification task may be implemented to each consist of one convolutional followed by one fully connected layer. However, we can further reduce the overheads associated with these two components.  Since convolutional layers consume more energy than fully connected layers \cite{eyerissenergy}, in order to further reduce hardware overhead, we can completely eliminate the convolutional layer in LE and GN by extracting useful features from GE. To do this feature extraction, instead of feeding input images directly to LE and GN, we can feed the outputs of one convolutional layer of GE to LE and GN. Thus, by reusing a convolutional layer of GE, storage and computation overheads of LE and GN can be reduced. Moreover, since GE is trained with large size generic dataset, its convolutional layers serve as very good feature extractors. Also because both generic and customized data are images of the same set of classes and they share some fundamental properties, the extracted features are actually good input to LE and GN. Note that despite this extraction, during the training of LE and GN, only the layers that exclusively belong to LE or GN are trained. %because we assume there is no access to the layers in GE.

Despite the above improvement, the size of the extracted feature maps  from GE may still be large, which makes the subsequent fully connected layer in LE or GN to also become large. For example, as we discuss in our experiments, the size of the first convolutional layer in GE is $12\times 12\times 20$ which results in a large fully-connected layer in LE and GN. To reduce the overheads associated with the fully connected layers in LE and GN, we need to reduce the size of the input feature maps while still preserving useful information.

To address the above challenge, we propose to use max pooling layer in LE and GN to further reduce the width and height of the input feature maps, then feed the sub-sampled feature maps to subsequent fully connected layer. This approach treats each feature map equally and is easy to implement. Another approach is to analyze the extracted features over many input data and then select the representative ones to be fed to subsequent fully connected layer. The above approaches are orthogonal and may be used together.

To complete the design of LE and GN we still need to determine the layer of GE whose output should be forwarded to LE and GN, as well as the extent the input feature maps should be sub-sampled. We note that LE and GN could have different answers for both of these questions and these answers are task-specific. For each task, these answers form the solution space that need to be explored to understand the tradeoff between overall performance and hardware overheads. Fortunately, LE and GN can be trained and tested independently, and the training of LE and GN are very fast due to small model and dataset. Finally, the configuration that provides good overall accuracy while incurs minimum hardware overhead is selected to be the final MOE architecture.
We discuss the above design considerations in detail in our experiments.

\vspace{-3mm}
\subsection{Effectiveness of LE \& Its Training Options}\vspace{-1mm}


Let us assume that GN is perfect in the sense that it will always select the correct output from either GE or LE, assuming correct output can be identified by one of the two. Then the real value of LE in terms of improving overall performance is its ability to correctly classify those samples that cannot be correctly classified by GE. In other words, the improvement of overall performance is determined by how well LE is able to complement GE.

Fig. \ref{fig:set} is a conceptual illustration that shows the sample regions covered by GE and LE. The outermost rectangle ($R1+R2+R3+R4$) represents all customized samples. $R1+R3$ represents the samples that can be correctly classified by GE. $R1+R2$ represents the samples that can be correctly classified by LE. $R4$ represents the samples that cannot be correctly identified by both GE and LE. The ability of LE to complement GE is shown by the relative size between $R2$ and $R4$. If $R2$ is much larger than $R4$, it indicates that LE is able to provide correct predictions on those samples that GE cannot handle, and LE complements GE very well. The overall performance is greatly improved in this case because only the samples in $R4$ cannot be correctly classified now, compared to that of $R2+R4$ originally.

In order to make LE maximally complement GE, we would like to directly train LE with samples in $R2+R4$ and train GN to distinguish samples in $R1+R3$ versus samples in $R2+R4$. However, our training experiences showed overfitting issue may occur due to insufficient training samples in $R2+R4$. %The details of this training setting has been explained in the second last paragraph of Section \ref{sec:threecomponents}.
Thus, when the size of customized data is limited, we train LE on all customized data and train GN to predict if an input data is customized or generic. Surprisingly, under this training setting, we observed that LE still complements GE very well. Overtime, when the number of customized data becomes large, we could easily switch back to the first training setting.
\begin{figure}[t]
        \centering
        \includegraphics[width=2in]{figs/set.pdf}\vspace{-2mm}
        \caption{Diagram of the sample region covered by GE and LE. Region $R1+R3$ represents the samples that can already be correctly classified by GE. Region $R2$ represents the samples that can \textit{only} be correctly classified by LE. It it one way to determine how well LE can complement GE.}\vspace{-7mm}
        \label{fig:set}
\end{figure}


==> prototype.tex <==
\section{Prototype}\label{sec:prototype}

